Near-Optimal Pure Exploration in Matrix Games: A Generalization of Stochastic Bandits & Dueling Bandits

We study the sample complexity of identifying the pure strategy Nash equilibrium (PSNE) in a two-player zero-sum matrix game with noise. Formally, we are given a stochastic model where any learner can sample an entry $(i,j)$ of the input matrix $A\in[-1,1]^{n\times m}$ and observe $A_{i,j}+\eta$ where $\eta$ is a zero-mean 1-sub-Gaussian noise. The aim of the learner is to identify the PSNE of $A$, whenever it exists, with high probability while taking as few samples as possible. Zhou et al. (2017) presents an instance-dependent sample complexity lower bound that depends only on the entries in the row and column in which the PSNE lies. We design a near-optimal algorithm whose sample complexity matches the lower bound, up to log factors. The problem of identifying the PSNE also generalizes the problem of pure exploration in stochastic multi-armed bandits and dueling bandits, and our result matches the optimal bounds, up to log factors, in both the settings.

==> discussion.tex <==
\section{{Conclusion and Open Questions}}
%\arnab{need to modify this section}
This paper characterizes the query complexity of finding the unique Nash equilibrium $(\xstar,\ystar)$ in two-player zero-sum matrix games. However, many interesting open questions remain. %Recall that in Theorem \ref{thm:psne}, we showed an $O(n\cdot \log(\frac{n}{\delta}))$ query complexity algorithm that finds the unique PSNE with probability at least $1-\delta$. We conjecture that the expected query complexity can be reduced to $O(n\log\log n)$. 
We showed in Theorem \ref{thm:mixed} that  with probability at least $1-\delta$, we can find $(\xstar,\ystar)$  by querying at most $O(nk^4\cdot\polylog(\frac{n}{\delta}))$ entries where $k=|\supp(\xstar)|$. In Theorem \ref{thm:lower-bound:new}, we showed a lower bound of $\Omega(nk)$. We conjecture that the upper and lower bound can be improved to $O(nk^2\cdot \polylog( \frac{n}{\delta}))$ and $\Omega(nk^2)$ respectively. 

Also, observe that our algorithm does not run in polynomial time as it is a support-enumeration based algorithm. In this case, designing a polynomial time randomized algorithm that takes $o(n^2)$ queries and finds the unique Nash equilibrium is also an interesting open question.  

Finally, recall that we depicted a deterministic algorithm with a query complexity of $O(n)$ to find the unique PSNE. We conjecture that if $|\supp(\xstar)|\geq 2$, then any deterministic algorithm takes $\Omega(n^2)$ queries to find the unique Nash equilibrium.





